This Prompt is Measuring <MASK>: Evaluating Bias Evaluation in Language Models

Bias research in NLP seeks to analyse models for social biases, thus helping NLP practitioners uncover, measure, and mitigate social harms. We analyse the body of work that uses prompts and templates to assess bias in language models. We draw on a measurement modelling framework to create a taxonomy of attributes that capture what a bias test aims to measure and how that measurement is carried out. By applying this taxonomy to 90 bias tests, we illustrate qualitatively and quantitatively that core aspects of bias test conceptualisations and operationalisations are frequently unstated or ambiguous, carry implicit assumptions, or be mismatched. Our analysis illuminates the scope of possible bias types the field is able to measure, and reveals types that are as yet under-researched. We offer guidance to enable the community to explore a wider section of the possible bias space, and to better close the gap between desired outcomes and experimental design, both for bias and for evaluating language models more broadly.

==> tables/taxonomy_table.tex <==
\begin{table*}[ht]
\begin{adjustbox}{width=1\textwidth}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{Prompt Task}    & \textbf{Use Context}  \\
sequence scoring, single word generation, \\
prompt continuation, full sentence response & zero-shot/few-shot, upstream LM, dialogue, Q\&A    \\
\midrule
\textbf{Conceptualisation}    & \textbf{Operationalisation}  \\ 
\midrule
stereotyping, toxic content generation, other, unclear     & \begin{tabular}[c]{@{}l@{}}output content assessed, output quality assessed,\\ difference in probability rank over fixed set, difference in output distributions,\\ most probable option/N options, difference in regard,\\ difference in sentiment, difference in toxicity\end{tabular} \\
\midrule
\textbf{Desired Outcome} & \textbf{Proxy Type} \\
\midrule
\begin{tabular}[c]{@{}l@{}}no impact of demographic term, negative stereotype not in model,\\ no harmful output generated, other, unclear\end{tabular} & \begin{tabular}[c]{@{}l@{}}identity terms, pronouns, names, roles,\\ associated words, dialect features,other, unclear\end{tabular}  \\
\midrule
\textbf{Demographic }      & \textbf{Gender Scope }   \\ 
\midrule
gender, religion, sexual orientation, ethnicity/race, other   & binary, binary + ack, binary + other, other only  \\
\midrule
\textbf{Prompt Origin} & \\
\midrule
author, crowd-sourced, corpus, auto generated & \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Taxonomy (not entire, but major categories. Can add the binary questions that aren't here like fixed set, language, etc?}
    % \label{tab:taxonomy}
\end{table*}
